Multispectral Image Segmentation in Agriculture: A Comprehensive Study on Fusion Approaches

Multispectral imagery is frequently incorporated into agricultural tasks, providing valuable support for applications such as image segmentation, crop monitoring, field robotics, and yield estimation. From an image segmentation perspective, multispectral cameras can provide rich spectral information, helping with noise reduction and feature extraction. As such, this paper concentrates on the use of fusion approaches to enhance the segmentation process in agricultural applications. More specifically, in this work, we compare different fusion approaches by combining RGB and NDVI as inputs for crop row detection, which can be useful in autonomous robots operating in the field. The inputs are used individually as well as combined at different times of the process (early and late fusion) to perform classical and DL-based semantic segmentation. In this study, two agriculture-related datasets are subjected to analysis using both deep learning (DL)-based and classical segmentation methodologies. The experiments reveal that classical segmentation methods, utilizing techniques such as edge detection and thresholding, can effectively compete with DL-based algorithms, particularly in tasks requiring precise foreground-background separation. This suggests that traditional methods retain their efficacy in certain specialized applications within the agricultural domain. Moreover, among the fusion strategies examined, late fusion emerges as the most robust approach, demonstrating superiority in adaptability and effectiveness across varying segmentation scenarios. The dataset and code is available at https://github.com/Cybonic/MISAgriculture.git.

==> backup.tex <==
\begin{table}[ht]
\centering
{\renewcommand{\arraystretch}{1.4}% for the vertical padding
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|c|ccccc}
\hline
Fusion &\textbf{Modality}  & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} & \textbf{IoU} \\ \hline
 & RGB & 75.04\% & 27.05\% & 32.82\% & 28.31\% & 16.72\%  \\
 & NVDI & 76.42\% & 31.7\% & 38.12\% & 32.89\% & 20.02\% \\ \hline \hline
\multirow{4}{*}{\rotatebox[origin=l]{90}{Late Fusion}} & \begin{tabular}[c]{@{}c@{}} RGB+NVDI\\ (Pixel-wise addition)\end{tabular} & 68.32\% &  26.68\% &  53.5\% & 34.2\% & 21.05\% \\
& \begin{tabular}[c]{@{}c@{}}RGB+NVDI\\ (Average)\end{tabular} & 68.32\%  & 26.68\% & 53.5\% & 34.2\% & 21.05\% \\ \hline \hline
\end{tabular}
\end{adjustbox}
}
\caption{Mean Classical Metrics Results}
\label{tab3}
\end{table}



\begin{table}[ht]
\centering
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
%\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l|l|ccccc}
\hline
\textbf{Method} &
  \multicolumn{1}{c|}{\textbf{Input}} &
  \textbf{Accuracy} &
  \textbf{Precision} &
  \textbf{Recall} &
  \textbf{F1 Score} &
  \textbf{IoU} \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Otsu's\\ Thresholding~\tablefootnote{\href{https://docs.opencv.org/4.x/d7/d4d/tutorial_py_thresholding.html}{OpenCV Image Thresholding}}\end{tabular}} &
  RGB &
  74.45 &
  26.56 &
  33.73 &
  28.32 &
  16.73 \\
 & NDVI           & 76.07 & 31.45 & 37.79 & 32.32 & 19.63 \\ \cline{2-7} 
 & Early Fusion & \multicolumn{5}{c}{\textbf{}}         \\
 & Average        & 75.63 & 30.81 & 41.85 & 34.09 & 20.94 \\ \cline{2-7} 
 & Late Fusion  & \multicolumn{5}{c}{\textbf{}}         \\
 & Average        & 67.49 & 26.24 & 54.03 & 33.73 & 20.76 \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Edge-based \\ Segmentation\tablefootnote{{\label{same}\href{https://scikit-image.org/docs/stable/auto_examples/applications/plot_coins_segmentation.html}{Comparing edge-based and region-based segmentation}}}\end{tabular}} &
  RGB &
  76.60 &
  15.53 &
  11.62 &
  12.90 &
  6.93 \\
 & NDVI           & 75.63 & 14.83 & 12.27 & 13.01 & 6.99  \\ \cline{2-7} 
 & Early Fusion & \multicolumn{5}{c}{\textbf{}}         \\
 & Average        & 70.08 & 13.01 & 16.45 & 14.03 & 7.58  \\ \cline{2-7} 
 & Late Fusion  & \multicolumn{5}{c}{\textbf{}}         \\
 & Average        & 69.19 & 15.24 & 21.94 & 17.46 & 9.62  \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Region-based\\ Segmentation\footref{same}\end{tabular}} &
  RGB &
  84.06 &
  44.30 &
  14.37 &
  21.00 &
  11.94 \\
 & NDVI           & 82.20  & 28.69 & 8.38  & 12.44 & 6.67  \\ \cline{2-7} 
 & Early Fusion & \multicolumn{5}{c}{\textbf{}}         \\
 & Average        & 76.66 & 21.52 & 18.53 & 18.95 & 10.54 \\ \cline{2-7} 
 & Late Fusion  & \multicolumn{5}{c}{\textbf{}}         \\
 & Average        & 81.81 & 35.65 & 20.61 & 25.28 & 14.71 \\ \hline
\end{tabular}
\caption{Mean classical metrics using three different classical methods.}
\label{tab:classic-vg}}
\end{table}



{p{0.2\columnwidth}|p{0.1\columnwidth}p{0.1\columnwidth}p{0.1\columnwidth}|p{0.1\columnwidth}p{0.1\columnwidth}p{0.1\columnwidth}|p{0.1\columnwidth}p{0.1\columnwidth}p{0.1\columnwidth}}





\begin{table}[ht]
\centering
\caption{Segmentation performance using Otsu Threshold (OST)\tablefootnote{\label{foot1}\href{https://docs.opencv.org/4.x/d7/d4d/tutorial_py_thresholding.html}{OpenCV Image Thresholding - Otsu's thresholding.}}, Edge-based\tablefootnote{\label{foot}{\href{https://scikit-image.org/docs/stable/auto_examples/applications/plot_coins_segmentation.html}{Edge-based and Region-based segmentation - Canny edge-detector and  Watershed transform.}}} and Region-based$^{\ref{foot}}$ methods on the Maize (VG) and Vine (Qta. Baixo, ESAC and Valdoeiro) datasets. The performance scores are presented in percentage [\%]. The fusion was obtained by computing the pixel-wise average of the modalities.}
{\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{1.4pt}
\begin{tabularx}{\dimexpr\textwidth}{cc|ccc|ccc|ccc|ccc|ccc}
\hline \noalign{\hrule height 1pt}
& & \multicolumn{3}{c|}{Maize} & \multicolumn{9}{c|}{Vine} \\ \cline{3-14} 
\multicolumn{2}{l|}{\diagbox{\tiny{Method}}{\tiny{Dataset}}}
&\multicolumn{3}{c|}{VG} &
\multicolumn{3}{c|}{Qta. Baixo}  & 
\multicolumn{3}{c|}{ESAC} & 
\multicolumn{3}{c|}{Valdoeiro} &  \multicolumn{3}{c}{Average} \\ 
& & Acc. & F1 & IoU & Acc. & F1 & IoU & Acc. & F1 & IoU & Acc. & F1 & IoU 
& Acc. & F1 & IoU\\   \hline \noalign{\hrule height 1pt}
\multirow{4}{*}{\rotatebox[origin=l]{90}{OTS}} & 
RGB & 74.4 & 28.3 & 16.7 
& 57.6 & 41.9 & 27.6 
& 79.1 & 52.7 & 40.2 & 
74.5 & 38.6 & 26.0 &
71.4 &  40.4 & 27.6\\
& NDVI &76.1 & 32.3 & 19.6 %vg
& 84.1&  61.7&  46.1        %qb
& 65.6 & 49.7 & 34.8       %esac
& 92.4 & 67.8 & 56.0 &
79.6 &  52.9&  39.1\\  \cline{2-17}  %val
&  Early F. & 75.6 & 34.1& 20.9 
& 71.6 &52.7 &37.7
& 71.4 & 55.5 & 41.2
& 89.5 & 65.3 & 52.7&
77.1 & 51.9 &   38.1\\ 
& Late F.& 67.5 & 33.7 & 20.8 
& 83.0& 67.5& 44.7 
& 89.5&  66.8 & 42.9
& 91.6 & 81.6 &56.7 &
82.7 & 62.4 & 41.3\\  \hline \hline
\multirow{4}{*}{\rotatebox[origin=l]{90}{Edge-b.}} & RGB & 
76.6 & 12.9 & 6.9 %vg
& 69.8 & 15.5 & 8.5 %qb
& 78.1 & 26.3 & 15.4 %esac
& 86.9 & 22.7 & 13.1 &
77.9 & 19.4 & 10.5\\
& NDVI & 75.6 &13.0 &7.0
& 70.3& 16.8 &9.3
& 61.1& 18.7& 10.4
&  94.2& 48.6 &33.7&
75.3 & 24.3 & 15.1 \\  \cline{2-17}
& Early F.&  84.1& 21.0& 11.9
& 76.8 &16.3& 8.9
& 65.4 &14.8 &8.0
& 93.9 &39.3 &25.8&
80.1& 22.9& 13.7 \\ 
& Late F.& 70.1 & 14.0 & 7.6
& 64.8 & 18.9 & 10.6
& 71.1& 25.5 & 14.8
& 87.6& 39.1& 25.1&
73.5 &24.4& 14.5\\  \hline \hline
\multirow{4}{*}{\rotatebox[origin=l]{90}{Region-b.}} & RGB & 
 84.1 & 21.0& 11.9
& 78.3& 47.4& 33.1
& 78.9& 44.3& 33.2
& 85.3& 44.6& 31.2&
81.7& 39.3& 27.4\\
& NDVI & 82.2& 12.4& 6.7
& 89.0& 67.9&  52.5
&  76.0& 50.9& 37.3
& 97.2& 76.3& 63.8&
86.1 & 51.9 & 40.1\\ \cline{2-17}
&  Early F. & 76.7& 19.0& 10.5
& 81.3 & 52.7& 37.0
& 87.6 & 63.5& 49.8
&  97.3& 77.6&  65.2 &
85.8 &53.2& 40.6\\ 
& Late F. & 81.8& 25.3& 14.7
&  93.1&  69.3& 34.9
&  92.1& 48.9& 24.6 
& 98.6&  82.7& 45.2&
91.4 &56.6 &29.9\\   \hline \noalign{\hrule height 1pt} %\hline 
\multirow{4}{*}{\rotatebox[origin=l]{90}{SegNet}} & 
RGB & 97.0 & 90.3 & 82.4 & 81.5 & 38.3 & 23.7 & 
81.8 & 51.1 & 34.6  & 
94.4 & 61.8 & 44.7 &
88.7 & 60.4 & 46.4 \\
& NDVI & 96.8 & 89.0 &  80.3 & 84.6 & 64.8 & 48.2 
&77.7 & 39.7 & 25.0 &  
92.9  &  50.9 & 34.2 & 
88.0 & 61.1 & 47.0 \\  \cline{2-17}
&  Early F. & 96.8 & 89.3 & 80.8 & 81.1 & 42.1 & 26.7 
& 81.4 & 50.5 & 33.9 & 
94.3 & 61.0 & 43.9 &
88.4 & 60.7 & 46.3 \\ 
& Late F. & 96.9 & 89.9 & 81.7 & 77.6 & 43.3 & 27.8 & 
91.9 &  79.6 & 66.2  &
91.6 & 64.0 & 47.1 &
89.5 & 65.0 & 55.7 \\  \hline \hline
\multirow{4}{*}{\rotatebox[origin=l]{90}{DeeplabV3}} & 
RGB & 97.3 & 89.2 & 81.1 & 
81.5 & 9.1 & 4.8 & 
78.3 & 4.5 & 2.5 & 
94.4 & 47.5 & 31.2 &
87.9 & 37.6 & 29.9\\
& NDVI &  97.2 & 88.4 & 80.1  &
85.9 & 44.1 & 22.8 & 
75.7 & 35.8 & 22.3 &   
92.5 & 4.1 & 2.1 &  
87.8 & 44.9 & 31.8\\  \cline{2-17}
&  Early F. & 97.3 & 89.2 & 81.2 & 
79.3 & 26.6 & 17.1 &  
79.1 & 20.2 & 12.4 &  
93.2 & 35.7 & 23.8 & 
87.2 & 42.9 & 33.6\\ 
& Late F.  & 97.4 & 89.6 & 81.7 &  
82.6 & 15.3 & 8.3 & 
78.9 &  17.3 & 11.1 &
93.9 & 40.3 & 25.9 &
88.2 & 40.6 & 31.8 \\  \hline
%\multirow{4}{*}{\rotatebox[origin=l]{90}{Average}} & RGB 
%&  78.4& 20.7 & 11.8 
%& 68.6&  34.9&  23.1
%&  78.7&  41.1 &  29.6
%& 82.2 &  35.3&  23.4
%& 77.0 & 33.0 & 21.8\\
%& NDVI & 78.0& 19.2& 11.1  
%&   \textbf{81.1} & 48.8&  \textbf{36.0}
%&   67.6 & 39.8&  27.5
%&   \textbf{94.6}& 64.2&  \textbf{51.2}
%& 80.3 & 43.0 & \textbf{31.4} \\ \cline{2-17}
%& Early F.  &\textbf{78.8}&  \textbf{24.7}&  \textbf{14.4}
%& 76.6&  40.6&  27.9
%& 74.8&  44.6&  \textbf{33.0} 
%& 93.6 &  60.7&  47.9
%& 81.0 & 42.7 & 30.8\\
%& Late F. &  73.1&  24.3&  \textbf{14.4}
%& 80.3&  \textbf{51.9} &  30.1
%&  \textbf{84.2} &  \textbf{47.1} &  27.4
%& 92.6 &  \textbf{67.8}&  42.3
%& \textbf{82.5} &  \textbf{47.8} & 28.6 \\\hline 
\noalign{\hrule height 1pt}
\end{tabularx}
\label{tab:classical}}
\end{table}



\begin{table}[ht]
\caption{Segmentation performance using SegNet and DeeplabV3 on VG and Vine datasets. The performance scores are presented in percentage [\%]. The early fusion was obtained by concatenation and the late fusion by computing the pixel-wise average of the modalities.}
{\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{1.7pt}
\begin{tabularx}{\dimexpr\textwidth+5mm}{cc|ccc|ccc|ccc|ccc|ccc}
\hline \noalign{\hrule height 1pt}
& & \multicolumn{3}{c|}{Maize} & \multicolumn{9}{c|}{Vine} \\ \cline{3-14} 
\multicolumn{2}{l|}{\diagbox{\tiny{Method}}{\tiny{Dataset}}}
&\multicolumn{3}{c|}{VG} &
\multicolumn{3}{c|}{Qta. Baixo}  & 
\multicolumn{3}{c|}{ESAC} & 
\multicolumn{3}{c|}{Valdoeiro} &  \multicolumn{3}{c}{Average} \\ 
& & Acc. & F1 & IoU & Acc. & F1 & IoU & Acc. & F1 & IoU & Acc. & F1 & IoU 
& Acc. & F1 & IoU\\ \hline \hline
\multirow{4}{*}{\rotatebox[origin=l]{90}{SegNet}} & 
RGB & 97.0 & 90.3 & 82.4 & 81.5 & 38.3 & 23.7 & 
81.8 & 51.1 & 34.6  & 
94.4 & 61.8 & 44.7 &
88.7 & 60.4 & 46.4 \\
& NDVI & 96.8 & 89.0 &  80.3 & 84.6 & 64.8 & 48.2 
&77.7 & 39.7 & 25.0 &  
92.9  &  50.9 & 34.2 & 
88.0 & 61.1 & 47.0 \\  \cline{2-17}
&  Early F. & 96.8 & 89.3 & 80.8 & 81.1 & 42.1 & 26.7 
& 81.4 & 50.5 & 33.9 & 
94.3 & 61.0 & 43.9 &
88.4 & 60.7 & 46.3 \\ 
& Late F. & 96.9 & 89.9 & 81.7 & 77.6 & 43.3 & 27.8 & 
91.9 &  79.6 & 66.2  &
91.6 & 64.0 & 47.1 &
89.5 & 65.0 & 55.7 \\  \hline \hline
\multirow{4}{*}{\rotatebox[origin=l]{90}{DeeplabV3}} & 
RGB & 97.3 & 89.2 & 81.1 & 
81.5 & 9.1 & 4.8 & 
78.3 & 4.5 & 2.5 & 
94.4 & 47.5 & 31.2 &
87.9 & 37.6 & 29.9\\
& NDVI &  97.2 & 88.4 & 80.1  &
85.9 & 44.1 & 22.8 & 
75.7 & 35.8 & 22.3 &   
92.5 & 4.1 & 2.1 &  
87.8 & 44.9 & 31.8\\  \cline{2-17}
&  Early F. & 97.3 & 89.2 & 81.2 & 
79.3 & 26.6 & 17.1 &  
79.1 & 20.2 & 12.4 &  
93.2 & 35.7 & 23.8 & 
87.2 & 42.9 & 33.6\\ 
& Late F.  & 97.4 & 89.6 & 81.7 &  
82.6 & 15.3 & 8.3 & 
78.9 &  17.3 & 11.1 &
93.9 & 40.3 & 25.9 &
88.2 & 40.6 & 31.8 \\  \hline \hline
\multirow{4}{*}{\rotatebox[origin=l]{90}{Average}} & 
RGB &  
97.2& 89.7 & 81.8 & 
81.5&  23.7 & 14.3 & 
80.1 & 27.8 & 18.6 & 
94.4& 54.7 & 38.0 & 
88.3& 49.6 & 38.2 \\
& NDVI & 
97.0 & 88.7  & 80.2 & 
85.3 & 54.5 & 35.5 & 
76.7 & 37.8 & 23.7 & 
92.7 & 27.5 & 18.2 & 
87.9 & \textbf{53.0} & 39.6 \\  \cline{2-17}
&  Early F.  & 
97.1 & 89.3 & 81.0 &   
80.2 & 34.4 & 21.9 & 
80.3 &  35.4 & 23.2 & 
93.8 & 48.4 & 33.9 & 
87.8 & 51.8 & 40.0  \\
& Late F.  & 
97.2 & 89.8 & 81.7 &   
80.1 & 29.3 & 18.1 & 
85.4 & 48.5 & 38.7 & 
92.8 & 52.2 & 36.5 & 
\textbf{88.9} & 52.8 & \textbf{43.8} \\\hline 
\noalign{\hrule height 1pt}
\end{tabularx}
\label{tab:deep}}
\end{table}

==> tabela_antiga.tex <==
\begin{table}[ht]
\centering
{\renewcommand{\arraystretch}{1}% for the vertical padding
%\begin{adjustbox}{max width=\textwidth}
\begin{tabular*}{\textwidth}{
m{0.2\textwidth}|
m{0.15\textwidth} <{\centering}
m{0.15\textwidth} <{\centering}
m{0.15\textwidth} <{\centering}
m{0.15\textwidth}<{\centering}
>{\centering\arraybackslash}m{0.15\textwidth}}
\hline  \noalign{\hrule height 1pt}\toprule	
\textbf{Input}  & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} & \textbf{IoU} \\ \hline
 RGB & 75.04\% & 27.05\% & 32.82\% & 28.31\% & 16.72\%  \\
  NVDI & 76.42\% & 31.7\% & 38.12\% & 32.89\% & 20.02\% \\ \hline \hline 
(Early Fusion) & & & & \\
 Average &54.81\% &  15.56\% &  42.16\% & 21.8\% & 12.3\%\\
 RGB+NVDI &54.81\% &  15.55\% &  42.16\% & 21.8\% & 12.3\% \\ \hline \hline
(Late Fusion) & & & & \\
 Average & 68.32\% &  26.68\% &  53.5\% & 34.2\% & 21.05\% \\
 RGB+NVDI & 68.32\%  & 26.68\% & 53.5\% & 34.2\% & 21.05\% \\ \hline \hline

\noalign{\hrule height 1pt}\toprule	
\end{tabular*}
%\end{adjustbox}
}
\caption{Mean Classical Metrics Results}
\label{tab3}
\end{table}




\begin{figure}[ht]
\centering
\includegraphics[scale=0.45]{Figures/regionbased_rgb.jpg}
\hspace{0.1cm}
\includegraphics[scale=0.45]{Figures/regionbased_ndvi.jpg}
\hspace{0.1cm}
\includegraphics[scale=0.45]{Figures/regionbased_ndvi+rgb.jpg}
\caption{RGB, NDVI and RGB + NDVI segmented masks obtained through the Region-based segmentation, respectively.}
\label{fig:masks}
\end{figure}



\begin{figure}[ht]
\centering
\includegraphics[scale=0.45]{Figures/rgb.png}
\hspace{0.05cm}
\includegraphics[scale=0.45]{Figures/gray_rgb.png}
\hspace{0.05cm}
\includegraphics[scale=0.45]{Figures/ndvi_color.jpg}
\caption{RGB, Gray RGB and  NDVI images, respectively.}
\label{fig:base_img}
\end{figure}
